Low-Resource Machine Translation Training Curriculum Fit for Low-Resource Languages

We conduct an empirical study of neural machine translation (NMT) for truly low-resource languages, and propose a training curriculum fit for cases when both parallel training data and compute resource are lacking, reflecting the reality of most of the world's languages and the researchers working on these languages. Previously, unsupervised NMT, which employs back-translation (BT) and auto-encoding (AE) tasks has been shown barren for low-resource languages. We demonstrate that leveraging comparable data and code-switching as weak supervision, combined with BT and AE objectives, result in remarkable improvements for low-resource languages even when using only modest compute resources. The training curriculum proposed in this work achieves BLEU scores that improve over supervised NMT trained on the same backbone architecture by +12.2 BLEU for English to Gujarati and +3.7 BLEU for English to Kazakh, showcasing the potential of weakly-supervised NMT for the low-resource languages. When trained on supervised data, our training curriculum achieves a new state-of-the-art result on the Somali dataset (BLEU of 29.3 for Somali to English). We also observe that adding more time and GPUs to training can further improve performance, which underscores the importance of reporting compute resource usage in MT research.

==> _table5_old.tex <==
\begin{table*}[ht]
\small
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Method} & \textbf{en-gu} & \textbf{gu-en} & \textbf{en-kk}  & \textbf{kk-en}  & \textbf{en-so}  & \textbf{so-en}   \\ 
\hline
\multicolumn{7}{l}{\emph{Other methods}} \\ \hline
%\citet{liu2018context} & - & - & - & - & - & 25.36^2\\
Multilingual, Supervised, Google Translate & 31.4 & 26.2 & 23.1 & 28.9 & 22.7 & 27.7 \\
Multilingual, Supervised, mBART25$^2$ & 0.1 & 0.3 & 2.5 & 7.4 & - & - \\ 
Bilingual, Unsupervised$^1$ &0.6$^{*}$&0.6$^{*}$&0.8$^{*}$&2.0$^{*}$& - & - \\
Bilingual, Supervised &3.5$^{*1}$ & 9.9$^{*1}$ & 2.4$^{*1}$ & 10.3$^{*1}$ & - & 25.36$^3$ \\
Bilingual, Semi-supervised$^1$ & 4.0$^{*}$ & 14.2$^{*}$ & 3.1$^{*}$ & 12.5$^{*}$ & - & - \\
\hline
\multicolumn{7}{l}{\emph{Ours}} \\ \hline
% Bilingual, Unsupervised \emph{MLM} + (\emph{BT} + \emph{AE}) &0.44&0.31&1.11&1.60& 8.53 & 7.99 \\
Bilingual, Weakly-supervised \emph{MLM} + (\emph{BT} + \emph{MT})&  &   &   &   &   &   \\ 
Bilingual, Weakly-supervised (\emph{MLM} + \emph{TLM}) + (\emph{BT} + \emph{MT}) &18.05 & 14.51 & 4.06 & 5.65 & 9.06 & 10.33 \\
Bilingual, Unsupervised \emph{MLM} + (\emph{BT} + \emph{AE}) &0.44 & 0.31 & 1.11 & 1.60 & 8.53 & 7.99 \\ 
% \boxRight Weakly-supervised (\emph{BT} + \emph{MT}) &18.13 & 14.36 & 5.86 & 8.02 & 14.92 & 14.31\\
\boxRight Weakly-supervised (\emph{BT} + \emph{MT}) & 12.97 & 15.70 & 6.15 & 4.68 & 14.42 & 14.44 \\
% \boxSpace\boxRight 4 GPUs & 22.38 & 21.04 & 7.26 & 10.63 & 16.96&15.83\\
\boxSpace\boxRight 4 GPUs & 12.56 & 16.10 & 6.36 & 4.26 & 15.70 & 16.16 \\
\bottomrule
\end{tabular}}
\vspace*{-0.5em}
\caption{BLEU scores for previous supervised and unsupervised results from $^1$\citet{kim2020and} ($^*$report SacreBLEU), $^2$\citet{liu2020multilingual}, and  $^3$\citet{liu2018context} and our weakly-supervised models which leverage comparable data mined using lexical translations. Test and validation sets are from WMT19 for Gujarati and Kazakh and from \citet{tracey2019corpus} for Somali. \emph{MLM}, \emph{AE}, \emph{BT} and \emph{MT} stand for Masked Language Model, Auto-Encoding loss, Back Translation loss and Machine Translation loss, respectively. Bolded means best score. \emph{MT} and \emph{TLM} objectives use the best comparable data as paired data according to \cref{table:comparable_data}. Our models, except for the last row, use a single 32GB GPU. For completeness sake, \citet{lakew2020low} reports supervised results for Somali on a pooled test set from sources that doesn't include the test corpus studied here. They achieve 9.16 and 13.38 for en-so and so-en, respectively.}
\vspace{-2mm}
\label{table:benchmark}
\vspace{-0.5em}
\end{table*}
